Active Switching: Packet Steering Flow Annotations

Our previous experience building systems for middlebox chain composition and scaling in software-defined networks has revealed that existing mechanisms of flow annotation commonly do not survive middlebox-traversals, or suffer from extreme identifier domain limitations resulting in excessive flow table size. In this paper, we analyze the structural artifacts resulting in these challenges, and offer a framework for describing the behavior of middleboxes based on actions taken on traversing packets. We then present a novel mechanism for flow annotation that features an identifier domain significantly larger than existing techniques, that is transparent to hosts traversed, and that conserves flow-table resources by requiring only a small number of match rules and actions in most switches. We evaluate said technique, showing that it requires less per-switch state than conventional techniques. We then describe extensions allowing implementation of this architecture within a broader class of systems. Finally, we close with architectural suggestions for enabling straightforward integration of middleboxes within software-defined networks.

==> motivation.tex <==
% Copyright © 2013 Saul St. John <sstjohn@cs.wisc.edu>
% All rights reserved

\section{Definitions and Assumptions}
\label{sec:motivation}

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\textwidth]{fabric}
\caption{Abstract network topology}
\label{fig:fabric}
\end{figure}
\begin{figure*}[ht!]
\centering
\includegraphics[width=0.8\textwidth]{chain}
\caption{Example policy chain}
\label{fig:policy_chain}
\end{figure*}


For the purposes of this system, we define a middlebox as a network device
that performs some application-level functionality. We employ a convenient
abstraction in this work, that all middleboxes have exactly
three interfaces:
\begin{compactitem}
\item An \textbf{ingress interface}, upon which traffic is only received.
\item A \textbf{egress interface}, upon which traffic is only transmitted.
\item A \textbf{control interface}, responsible for management traffic.
\end{compactitem}
We do not believe that this abstraction in any way lessens the generality
of the discussion to follow. Consider another occasionally-useful
abstraction of interfaces, which we employ in later sections:
\begin{compactitem}
\item An \textbf{upstream interface}, upon which traffic originating from
	the external network is received, and through which traffic 
	originating from endpoint hosts within the network is transmitted.
\item A \textbf{downstream interface}, which functions as the inverse of 
	the upstream interface.
\item A \textbf{control interface}, as in the previous abstraction.
\end{compactitem}
These abstractions are equivalent, as the following construction demonstrates:
on a middlebox featuring physical upstream/downstream interfaces, the abstract
ingress interface traffic can be identified as that which is received by either
physical interface. Conversely, the abstract egress interface traffic is 
necessarily all traffic transmitted by either physical interface. The control
interface behaves identically under either abstraction.

We assume the existence of a network fabric as described by 
M.~Casado,~\textit{et al.}in \cite{fabric}, with OpenFlow-enabled
edge switches. Positioned about the fabric is a collection of servers, 
middleboxes, and gateway switches connecting to an external network. This 
abstract topology is illustrated by Figure \ref{fig:fabric}, where the numerals
situated about the fabric identify the egress port from the network for traffic
bound for a particular device.\footnote{In later sections, we show that the
fabric abstraction is equivalent to a connected graph of OpenFlow-enabled
switches with a common controller. As such, this abstraction does not limit 
the generality or applicability of the discussion to follow.}
The figure omits, and we do not define identifiers for, the fabric's ingress
ports.

Multiple tenants may co-exist within this network; as such, the various endpoints
may not share a common owner, and their connectivity may be logically isolated
from that of other tenants within the same network by means of a network 
virtualization facility such as 802.1q~\cite{802.1q}, STT~\cite{stt}, 
VXLAN~\cite{vxlan} or NVGRE~\cite{nvgre}.

We further assume a policy language for describing rules interposing chains 
of middleboxes between the ingress switch and destination for traffic matching 
given patterns, and an OpenFlow controller, connected to the fabric's edge 
switches.

We will consider, as an example, a policy that specifies traffic destined for
host \textit{H} must first traverse one of two redundancy eliminators 
\textit{RE1} or \textit{RE2}, followed by a single intrusion prevention device
\textit{IPS}. This policy is illustrated in Figure \ref{fig:policy_chain}.

We further specify two general requirements on the behavior of the
system:
\begin{compactitem}
\item A flow initially submitted to one of multiple potential equivalent 
middleboxes must maintain \textbf{affinity} with that instance over the life 
of the flow.
\item A flow that passes through a given sequence of middleboxes on the 
downstream path to the destination must maintain \textbf{symmetricality} on
the return path, meaning that the very same middleboxes must be traversed in
reverse order.
\end{compactitem}

We now consider the question of how such a controller might program the edge 
switches of the fabric to effect this policy.



==> sources.tex <==
% Copyright © 2013 Saul St. John <sstjohn@cs.wisc.edu>
% All rights reserved

\subsubsection*{Source}
The active switching proof-of-concept implementation (called SOFT) can be found at 
\url{http://pages.cs.wisc.edu/~sstjohn/soft.tgz}. It
is released under the terms of the GPLv3.


==> taxonomy.tex <==
% Copyright © 2013 Saul St. John <sstjohn@cs.wisc.edu>
% All rights reserved

\section{Taxonomy}
For reasons historical, there are two
predominant architectural foundations upon which the higher-level functionality
of middleboxes is implemented. In general, the distinction between these
types of middleboxes can be distinguished by the type of traffic the middlebox
is able to "see":
\begin{compactitem}
\item A \textbf{bridging middlebox} receives all packets available on the
medium.
\item A \textbf{routing middlebox} only receives packets that are constructed so
as to appear that the middlebox is a valid "next-hop" on a
route from the source address to the destination address, given the middlebox's
IP configuration.
\end{compactitem}

While this distinction implies the potential side-effects of a
given middlebox, it's important to note that it does not meaningfully describe or
constrain the behavior a given middlebox may exhibit with respect to traffic
"seen". For the purpose of discussing the behavior and higher-level 
functionality 
implemented by a middlebox, this distinction is not useful, as these types
of middlebox are roughly equipotent.

To the end of describing the behavior of middleboxes from the perspective of
the network itself, we can also classify middleboxes based on their possible
behavior \textit{upon those packets received}:
\begin{compactitem}
\item A \textbf{transparent middlebox} emits all packets received from upstream
without alteration in the downstream direction.
\item A \textbf{translucent middlebox} need not emit all packets, but all packets
that are emitted in the downstream direction are identical to
some packet received from upstream.
\item A \textbf{mangling middlebox} may emit packets downstream
that are not identical to some packet received from upstream; however, each packet 
emitted downstream "corresponds"\footnote{This relationship is left vague somewhat intentionally, as
a middlebox which appears to originate and terminate flows when considered as a black-box may, 
in fact, be recognizable as a mangling middlebox given a sufficiently 
nuanced understanding of its behavior.} to some packet received from upstream.
\item A \textbf{connection-originating middlebox} may act as an originator of
new flows.
\item A \textbf{connection-terminating middlebox} may terminate flows received.\footnote{This could also be viewed
as an extreme case of middlebox translucency.} 
\end{compactitem}

We will be using this latter terminology to describe middleboxes through which
traffic might be steered throughout the rest of the paper.\footnote{Only a
subset of this taxonomy is employed in the remainder, as only that subset
is relevant to the design of active switching. We believe though that this 
taxonomy, as a whole, could have broader utility for related middlebox 
research, and offer it to that end.}

